WikiAutoGen: Towards Multi-Modal Wikipedia-Style Article Generation

Knowledge discovery and collection are intelligence-intensive tasks that traditionally require significant human effort to ensure high-quality outputs. Recent research has explored multi-agent frameworks for automating Wikipedia-style article generation by retrieving and synthesizing information from the internet. However, these methods primarily focus on text-only generation, overlooking the importance of multimodal content in enhancing informativeness and engagement. In this work, we introduce WikiAutoGen, a novel system for automated multimodal Wikipedia-style article generation. Unlike prior approaches, WikiAutoGen retrieves and integrates relevant images alongside text, enriching both the depth and visual appeal of generated content. To further improve factual accuracy and comprehensiveness, we propose a multi-perspective self-reflection mechanism, which critically assesses retrieved content from diverse viewpoints to enhance reliability, breadth, and coherence, etc. Additionally, we introduce WikiSeek, a benchmark comprising Wikipedia articles with topics paired with both textual and image-based representations, designed to evaluate multimodal knowledge generation on more challenging topics. Experimental results show that WikiAutoGen outperforms previous methods by 8%-29% on our WikiSeek benchmark, producing more accurate, coherent, and visually enriched Wikipedia-style articles. Our code and examples are available at https://wikiautogen.github.io/

==> Tabletex/ablation-hard.tex <==
\begin{table*}[htbp]
\label{ablation-hard}
\centering
\vspace{-3mm}
\fontsize{8pt}{10pt}\selectfont
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c c c c c c c c c c c c@{}}
\toprule
 & \multirow{3}{*}{\textbf{Methods}} & \multicolumn{4}{c}{\textbf{Content Quality}}  & \multicolumn{2}{c}{\textbf{Informativeness}} & \multicolumn{1}{c}{\textbf{Reliability}} &
 \multicolumn{2}{c}{\textbf{Engagement}} 
 & \multirow{2}{*}{\textbf{Average}}
\\
\cmidrule(lr){3-6} \cmidrule(lr){7-8} 
\cmidrule(lr){9-9} 
\cmidrule(lr){10-11} 
&  & {\textit{\textbf{Alignment}}}  & {\textit{\textbf{Consistency}}} & {\textit{\textbf{Relevance}}} & {\textit{\textbf{Repetition}}} & {\textit{\textbf{Breadth}}}  & {\textit{\textbf{Depth}}} & {\textit{\textbf{Verifiability}}}  & {\textit{\textbf{Engagement}}} & {\textit{\textbf{Novelty}}}   \\
\cmidrule{1-12}
\multicolumn{12}{c}{\cellcolor{grayred} \textbf{\textit{WikiSeek-Ex}}} \\
\cmidrule{1-12}
& Storm  & 68.40 & 74.88 & 70.45 & 65.95&  64.72 & 59.26 & 51.21  & 58.84  & 53.316 & 63.00 \\
& OmniThink & 69.96 & 79.24 & 70.75 & 68.12 & 61.88 & 60.76 &46.55  & 55.97  &52.97  & 62.91 \\
& Ours  & 79.33 & 89.68  & 89.78 &79.1& 81.93  &  72.05& 72.32 & 71.41  & 69.50 & 78.35 \\
\cmidrule{1-12}
\multicolumn{12}{c}{\cellcolor{uclagold} \textbf{\textit{WikiSeek-V}}} \\
\cmidrule{1-12}
& Storm  & 75.88 & 82.59 & 70.58 & 72.24 & 65.03   & 65.53 & 51.77 & 57.95  & 57.72 &  66.58 \\
& OmniThink & 72.19 & 80.71 & 75.54 & 71.07 &  66.21 & 62.62 & 50.78  & 57.21  &54.35  & 65.63 \\
& Ours  & 83.65 & 91.98  & 89.34  &84.81 & 78.16  & 71.95 & 71.37 & 74.17  &68.52  &  79.33 \\
\cmidrule{1-12}
\multicolumn{12}{c}{\cellcolor{uclablue} \textbf{\textit{WikiSeek-H}}} \\
\cmidrule{1-12}
& Storm  & 73.20 & 79.92  & 72.63 & 70.20& 67.12  & 63.0  &54.26  & 59.62  & 55.71 &  66.18 \\
& OmniThink &  69.42& 79.06 & 70.95 & 68.60 & 62.58  & 60.26 &  48.37& 58.99  & 52.32 &63.39  \\
& Ours  & 82.08 & 90.94 & 84.93 &86.94 & 78.85  & 77.17 & 68.41 & 67.83  &69.6  &  78.53 \\
\bottomrule
\end{tabular}}
\caption{Quantitative comparisons.}
% \vspace{-5mm}
\end{table*}

==> Tabletex/ablation1.tex <==
\begin{table*}[t]
\label{ablation}
\vspace{-8mm}
\centering
\caption{Ablation studies in VL-WikiSeek-H.}
\vspace{-3mm}
\fontsize{8pt}{10pt}\selectfont
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c c c c c c c c c c c c c c@{}}
\toprule
\multicolumn{3}{c}{\textbf{Modules}}   & \multicolumn{3}{c}{\textbf{Comprehensibility}}  & \multicolumn{4}{c}{\textbf{Comprehensibility}} & \multicolumn{2}{c}{\textbf{ Captivatingness}} 
\\
\cmidrule(lr){1-3}  \cmidrule(lr){4-6} \cmidrule(lr){7-10} \cmidrule(lr){11-13} 
{\textit{\textbf{Rewrite}}} & {\textit{\textbf{Multi-agent}}} & {\textit{\textbf{Self-doubt}}}   & {\textit{\textbf{Alignment}}} & {\textit{\textbf{Relevance}}} & {\textit{\textbf{Repetition}}} & {\textit{\textbf{Breadth}}}  & {\textit{\textbf{Consistency}}} & {\textit{\textbf{Depth}}} & {\textit{\textbf{Verifiability}}}  & {\textit{\textbf{Engagement}}} & {\textit{\textbf{Novelty}}}   \\
\cmidrule{1-13}
\multicolumn{13}{c}{\cellcolor{grayred} \textbf{\textit{Text-Only Input}}} \\
\cmidrule{1-13}
 \usym{1F5F6}   &  \usym{1F5F6}  & \usym{1F5F6} & 79.35 &  79.92 & 77.57 & 72.21 & 86.836 & 68.97 & 64.45  & 62.68  & 60.37     \\
 \usym{2714}   &  \usym{1F5F6}  & \usym{1F5F6} & 60.7 &  62.03 & 62.92 &  57.12 & 77.9 & 55.31   & 52.148 & 53.73  &  48.88  \\
 \usym{1F5F6}   & \usym{2714}   & \usym{1F5F6}  & 75.22 & 74.60  & 67.20  & 68.12  & 79.92 & 62.75  &59.29  & 61.62 &  65.70\\
\usym{1F5F6}   & \usym{1F5F6}   & \usym{2714}  & 78.08 &  83.93 & 76.94 & 74.85  & 84.94 & 68.17 & 66.4 & 63.83  &  59.6     \\
\usym{2714}  & \usym{2714}  & \usym{2714}  & 82.08 & 84.93  & 86.94 & 78.85  & 90.94 & 77.17 & 68.40 &  67.83 & 69.60        \\
\cmidrule{1-13}
\multicolumn{13}{c}{\cellcolor{uclagold} \textbf{\textit{Image-Only Input}}} \\
\cmidrule{1-13}
 \usym{1F5F6}   &  \usym{1F5F6}  & \usym{1F5F6}    & 54.40   & 55.91  & 55.21 & 51.13  & 66.91 & 47.82 & 46.51 & 47.31  & 41.98    \\
 \usym{2714}   &  \usym{1F5F6}  & \usym{1F5F6}    & 79.85 &  81.38 & 77.39 & 73.15 & 87.09 & 69.55  & 65.59   & 64.25  & 62.06   \\
 \usym{1F5F6}   & \usym{2714}   & \usym{1F5F6}   & 76.35 & 76.36  & 66.95 &  61.68 & 71.02 & 60.28 & 65.56 & 61.49   & 55.09     &   \\
\usym{1F5F6}   & \usym{1F5F6}   & \usym{2714}  &  76.69 & 82.28  & 76.11 & 73.45  & 84.41 & 67.29   & 67.16 & 62.65  & 58.86   \\
\usym{2714}  & \usym{2714}  & \usym{2714}  & 82.69 & 86.27  & 79.10 & 75.44  & 89.41 & 78.28 & 68.16 & 69.64  & 68.86       \\
\cmidrule{1-13}
\multicolumn{13}{c}{\cellcolor{uclablue} \textbf{\textit{Multi-modal Input}}} \\
\cmidrule{1-13}
 \usym{1F5F6}   &  \usym{1F5F6}  & \usym{1F5F6} & 75.82 & 77.25  & 74.71 & 70.14  & 85.77 & 65.87  & 61.69  &  61.72 &  57.89    \\
 \usym{2714}   &  \usym{1F5F6}  & \usym{1F5F6}    & 59.81 & 60.05 & 61.66  &  56.81 & 78.04 & 54.17  & 54.78 & 53.38  & 47.15     \\
 \usym{1F5F6}   & \usym{2714}   & \usym{1F5F6}   & 68.99 & 72.14  & 68.19   &  64.37 & 76.00 &  59.13 & 61.4 & 59.16  &  61.99    \\
\usym{1F5F6}   & \usym{1F5F6}   & \usym{2714}  &  77.47 & 84.46  & 76.57 &  75.74 & 84.42 & 67.79 & 68.26 & 64.10  & 59.45      \\
\usym{2714}  & \usym{2714}  & \usym{2714}  & 83.47 & 86.46  & 81.57  & 79.73  & 90.42 & 72.79   &70.26  & 66.17  & 69.45  \\
\bottomrule
\end{tabular}}
\vspace{-5mm}
\end{table*}


==> Tabletex/ablation2.tex <==
% \begin{table*}[t]
% \label{mainresult}
% \vspace{-8mm}
% \centering
% \caption{Ablation stduy. Info. Sup. means Information Supplementation, and Vis. Rein. means Visual Reinforcement.}
% \vspace{-3mm}
% \fontsize{8pt}{10pt}\selectfont
% \resizebox{0.9\linewidth}{!}{
% \begin{tabular}{@{}c c c c c c c c c c@{}}
% \toprule
%  & \multirow{3}{*}{\textbf{Methods}} & \multicolumn{6}{c}{\textbf{Multimodal Metrics}}   & 
%  & \multirow{2}{*}{\textbf{Average}}
% \\
% \cmidrule(lr){3-8} 
% &  & {\textit{\textbf{Coherence}}} & {\textit{\textbf{Engagement}}} & {\textit{\textbf{Helpfulness}}}  & {\textit{\textbf{Info. Sup.}}} & {\textit{\textbf{Relevance}}} & {\textit{\textbf{Vis. Rein.}}}   \\
% \cmidrule{1-10}
% \multicolumn{10}{c}{\cellcolor{grayred} \textbf{\textit{Text as Topic}}} \\
% \cmidrule{1-10}
% & Storm  &  55.20 & 45.97 & 51.89 & 43.97 & 54.07 & 48.86 &  49.99  \\ 
% & Co-Storm   & 57.62  & 48.64 & 54.19 & 45.07 & 55.87 & 50.48 &  51.98  \\
% & OmniThink  & 58.82  & 49.36 & 54.93 & 47.55 & 56.99 & 52.26 &  53.32  \\
% & Ours & 70.12  & 66.31 & 74.76 & 64.78 & 70.37 & 66.67 &  68.84  \\
% \cmidrule{1-10}
% \multicolumn{10}{c}{\cellcolor{uclagold} \textbf{\textit{Image as Topic}}} \\
% \cmidrule{1-10}
% & Storm  &  52.60 & 43.97 & 49.53 & 41.84 & 51.64 & 46.74 &  47.72  \\
% & Co-Storm   & 54.32  & 45.61 & 51.55 & 41.56 & 53.02 & 47.17 &   48.87 \\
% & OmniThink  & 59.87  & 50.61 & 56.12 & 47.23  & 57.31 & 52.31  &  53.90  \\
% & Ours & 71.90  & 61.69 & 77.63 & 63.88 & 69.21 & 68.22 &  68.76  \\
% \cmidrule{1-10}
% \multicolumn{10}{c}{\cellcolor{uclablue} \textbf{\textit{Image-Text as Topic}}} \\
% \cmidrule{1-10}
% & Storm  & 59.67  & 50.26 & 55.78 & 46.78 & 57.62 & 52.11 &  53.70  \\
% & Co-Storm   & 54.28  & 45.65 & 51.29 & 42.89  & 53.31 & 48.09 &  49.25  \\
% & OmniThink  &  61.76 & 51.40 & 57.88 & 49.97 & 59.83 & 54.88 &  55.95  \\
% & Ours & 72.24  & 70.29 & 72.11 & 69.29 & 66.77 & 66.29 &   69.50 \\
% \bottomrule
% \end{tabular}}
% \vspace{-5mm}
% \end{table*}



\begin{table*}[t]
\centering
\caption{Ablation study. Info. Sup. means Information Supplementation, and Vis. Rein. means Visual Reinforcement.}
\label{mainresult}
\vspace{-3mm}
\fontsize{8pt}{10pt}\selectfont
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{@{}c c c c c c c c c@{}}
\toprule
 & \multirow{3}{*}{\textbf{Methods}} & \multicolumn{6}{c}{\textbf{Multimodal Metrics}} & \multirow{3}{*}{\textbf{Average}} \\
\cmidrule(lr){3-8}
 &  & {\textit{\textbf{Coherence}}} & {\textit{\textbf{Engagement}}} & {\textit{\textbf{Helpfulness}}}  & {\textit{\textbf{Info. Sup.}}} & {\textit{\textbf{Relevance}}} & {\textit{\textbf{Vis. Rein.}}} &  \\
\cmidrule{1-9}
\multicolumn{9}{c}{\cellcolor{grayred} \textbf{\textit{Text as Topic}}} \\
\cmidrule{1-9}
 & Storm  &  55.20 & 45.97 & 51.89 & 43.97 & 54.07 & 48.86 &  49.99  \\ 
 & Co-Storm   & 57.62  & 48.64 & 54.19 & 45.07 & 55.87 & 50.48 &  51.98  \\
 & OmniThink  & 58.82  & 49.36 & 54.93 & 47.55 & 56.99 & 52.26 &  53.32  \\
 & Ours & 70.12  & 66.31 & 74.76 & 64.78 & 70.37 & 66.67 &  68.84  \\
\cmidrule{1-9}
\multicolumn{9}{c}{\cellcolor{uclagold} \textbf{\textit{Image as Topic}}} \\
\cmidrule{1-9}
 & Storm  &  52.60 & 43.97 & 49.53 & 41.84 & 51.64 & 46.74 &  47.72  \\
 & Co-Storm   & 54.32  & 45.61 & 51.55 & 41.56 & 53.02 & 47.17 &   48.87 \\
 & OmniThink  & 59.87  & 50.61 & 56.12 & 47.23  & 57.31 & 52.31  &  53.90  \\
 & Ours & 71.90  & 61.69 & 77.63 & 63.88 & 69.21 & 68.22 &  68.76  \\
\cmidrule{1-9}
\multicolumn{9}{c}{\cellcolor{uclablue} \textbf{\textit{Image-Text as Topic}}} \\
\cmidrule{1-9}
 & Storm  & 59.67  & 50.26 & 55.78 & 46.78 & 57.62 & 52.11 &  53.70  \\
 & Co-Storm   & 54.28  & 45.65 & 51.29 & 42.89  & 53.31 & 48.09 &  49.25  \\
 & OmniThink  & 61.76  & 51.40 & 57.88 & 49.97 & 59.83 & 54.88 &  55.95  \\
 & Ours & 72.24  & 70.29 & 72.11 & 69.29 & 66.77 & 66.29 &   69.50 \\
\bottomrule
\end{tabular}%
}
\vspace{-5mm}
\end{table*}

==> Tabletex/ablation3.tex <==
\begin{table*}[t]
\label{ablation-hard}
% \vspace{-8mm}
\centering
% \vspace{-3mm}
\fontsize{8pt}{10pt}\selectfont
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}c c c c c c c c c c c c@{}}
\toprule
 & \multirow{3}{*}{\textbf{Methods}} & \multicolumn{4}{c}{\textbf{Content Quality}}  & \multicolumn{2}{c}{\textbf{Informativeness}} & \multicolumn{1}{c}{\textbf{Reliability}} &
 \multicolumn{2}{c}{\textbf{Engagement}} 
 & \multirow{2}{*}{\textbf{Average}}
\\
\cmidrule(lr){3-6} \cmidrule(lr){7-8} 
\cmidrule(lr){9-9} 
\cmidrule(lr){10-11} 
&  & {\textit{\textbf{Alignment}}}  & {\textit{\textbf{Consistency}}} & {\textit{\textbf{Relevance}}} & {\textit{\textbf{Repetition}}} & {\textit{\textbf{Breadth}}}  & {\textit{\textbf{Depth}}} & {\textit{\textbf{Verifiability}}}  & {\textit{\textbf{Engagement}}} & {\textit{\textbf{Novelty}}}   \\
\cmidrule{1-12}
\multicolumn{12}{c}{\cellcolor{grayred} \textbf{\textit{WikiSeek-Ex}}} \\
\cmidrule{1-12}
% & Direct Gen &   &    &   &   &  &   &   &   &   &   \\
& oRAG & 58.85  &  75.40  & 74.05  &  73.00 & 60.97 & 50.99  & 40.51  & 56.10  & 44.06  & 59.33  \\
& Storm  & 68.40 & 74.89 & 70.45 & 65.95&  64.72 & 59.26 & 51.21  & 58.84  & 53.32 & 63.00 \\
& Co-Storm  &  79.16 &  84.14  & 74.12  & 75.23 & 67.95 & 66.85  & 57.15  & 60.28  & 61.44  & 69.59  \\
& OmniThink & 69.96 & 79.25 & 70.75 & 68.12 & 61.88 & 60.76 &46.55  & 57.21  &52.97  & 63.05 \\
& Ours  & 79.33 & 89.68  & 89.78 &79.10& 81.93  &  72.05& 72.32 & 71.41  & 69.50 & 78.34 \\
\cmidrule{1-12}
\multicolumn{12}{c}{\cellcolor{uclagold} \textbf{\textit{WikiSeek-V}}} \\
\cmidrule{1-12}
% & Direct Gen &   &    &   &   &   &   &   &   &   &   \\
& oRAG & 63.38  &  73.97  & 77.00  & 71.11 & 64.14 & 54.06  &  46.18 & 57.19  & 46.77  & 61.53  \\
& Storm  & 75.88 & 82.60 & 70.58 & 72.24 & 65.03   & 65.53 & 51.77 & 57.95  & 57.71 &  66.59 \\
& Co-Storm  & 77.15  &  83.84  & 75.57  & 74.91 & 69.03 & 67.82  & 58.75  & 61.73  & 61.27  &  70.01 \\
& OmniThink & 72.19 & 80.71 & 75.54 & 71.07 &  66.20 & 62.62 & 50.78  & 58.99  &54.35  & 65.83 \\
& Ours  & 83.64 & 91.98  & 89.34  &84.81 & 78.15  & 71.96 & 71.36 & 74.17  &68.52  &  79.33 \\
\cmidrule{1-12}
\multicolumn{12}{c}{\cellcolor{uclablue} \textbf{\textit{WikiSeek-H}}} \\
\cmidrule{1-12}
% & Direct Gen &   &    &   &   &   &   &   &   &   &   \\
& oRAG &  61.83 & 72.52   & 77.07  &  69.23 & 64.81 & 52.22  & 49.72  & 59.24  & 44.88  &  61.28 \\
& Storm  & 73.20 & 79.92  & 72.63 & 70.20& 67.12  & 63.05  &54.26  & 59.62  & 55.70 &  66.19 \\
& Co-Storm  &  77.83 &  84.33  & 75.65  &  76.05 & 68.29 & 68.43  & 58.69  & 61.04  &  62.13 &  70.27 \\
& OmniThink &  69.43 & 79.06 & 70.95 & 68.61 & 62.58  & 60.26 &  48.38 & 55.97  & 52.32 &63.06  \\
& Ours  & 82.08 & 90.94 & 84.93 &86.94 & 78.85  & 77.17 & 68.40 & 67.83  &69.60  &  78.53 \\
\bottomrule
\end{tabular}}
\caption{Quantitative comparisons.}
\vspace{-5mm}
\end{table*}

==> Tabletex/datastat.tex <==
\begin{table}[t]
  \vspace{-2mm}
  \centering
  \caption{The statistics of VL-WikiSeek.}
  \label{tab:statistics} 
  \resizebox{1.0\linewidth}{!}{ 
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Dataset} & \textbf{VL-WikiSeek-Ex} & \textbf{VL-WikiSeek-V} & \textbf{VL-WikiSeek-H} & \textbf{Overall} \\
    \midrule
    \textbf{Topics} & 3,992   &  126,066  &  49,452 & 179,510 \\
    \textbf{Images} & 4,457  &  160,684  &  75,237& 240,378 \\   
    \textbf{Single Image Topic} & 3,638  &  103,939  & 36,329 & 143,906 \\
    \textbf{Two Images Topic} & 297  &  16,218  & 7,725 & 24,240 \\
    \textbf{Three+ Images Topic}   & 57  &  5,909  & 5,398 & 11,364 \\
    \textbf{Vital-Booster Images} & 3,984  & 126,040   & 49,425 & 179,449 \\
    \textbf{Meta-rich Images}    & 106  &  26  & 27 & 61 \\
    \bottomrule
    \end{tabular}
  }
  \vspace{-6mm}
\end{table}


==> Tabletex/evaluator.tex <==
\begin{table}[htbp]
\centering
% \vspace{-0.3cm}
\resizebox{0.92\linewidth}{!}{
    \begin{tabular}{c l ccc ccc ccc c}
    \toprule
    \multirow{3}{*}{\textbf{Evaluator}} & \multirow{3}{*}{\textbf{Method}} 
    & \multicolumn{3}{c}{\textbf{Text as Topic}} 
    & \multicolumn{3}{c}{\textbf{Image as Topic}}  
    & \multicolumn{3}{c}{\textbf{Image-Text as Topic}} & \multirow{3}{*}{\textbf{Average}}  \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}  \cmidrule(lr){9-11}
    &  & Easy & Medium & Hard & Easy & Medium & Hard & Easy & Medium & Hard & \\
    \midrule
    \multirow{5}{*}{Gemini 2.5 Flash}   
    & oRAG         & 57.76 & 53.31 & 49.72 & 49.36 & 46.47 & 45.02 & 52.31 & 49.77 & 54.16 & 50.87\\
    & Storm        & 60.27 & 58.11 & 59.72 & 43.19 & 41.97 & 40.27 & 59.22 & 55.19 & 54.98  & 52.55\\
    & Co-Storm     & 59.31 & 63.21 & 50.02 & 44.32 & 45.01 & 43.67 & 64.02 & 62.15 & 59.63 & 54.59\\
    & OmniThink    & 52.15 & 55.31 & 47.02 & 39.29 & 41.74 & 41.21 & 54.02 & 56.22 & 51.73  & 48.63 \\
    \rowcolor{lightyellow}
    & \textbf{Ours}&\textbf{ 77.32} & \textbf{76.02} & \textbf{73.07} & \textbf{79.32} & \textbf{76.04} & \textbf{74.21} & \textbf{85.12} & \textbf{81.32} & \textbf{79.63} & \textbf{78.02}  \\
    \midrule
    \multirow{5}{*}{Prometheus2}   
    & oRAG         &65.25& 68.73 &59.53 &48.75 & 52.65 &46.25 & 69.36&  68.73& 61.72 & 60.11\\
    & Storm        &74.46 & 74.76  &74.34& 56.01& 64.51 &55.54 &73.08 & 69.55 & 69.36 & 67.96 \\
    & Co-Storm     &76.29 & 78.03 & 78.73& 63.11& 67.23& 63.42 & 75.78 &73.84 & 74.12 & 72.28 \\
    & OmniThink    &68.86 &69.25 & 64.22 &51.03 & 53.35 &51.23 &66.20 &60.32 & 60.50 & 60.55 \\
    \rowcolor{lightyellow}
    & \textbf{Ours} & \textbf{88.51} & \textbf{87.53} & \textbf{89.71}  & \textbf{89.07} &\textbf{89.53} & \textbf{90.03}  &\textbf{88.62}  & \textbf{89.26} & \textbf{88.79} & \textbf{89.01}  \\
    \bottomrule
    \end{tabular}
}
% \vspace{-0.3cm}
\caption{Results across different evaluators.}
\label{tab:evaluator}
% \vspace{-0.5cm}
\end{table}

==> Tabletex/mainresult1.tex <==
\begin{table*}[t]
\label{mainresult}
\vspace{-8mm}
\centering
\caption{Quantitative comparisons.}
\vspace{-3mm}
\fontsize{8pt}{10pt}\selectfont
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c c c c c c c c c c c c@{}}
\toprule
 & \multirow{3}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{Content Quality}}  & \multicolumn{2}{c}{\textbf{Informativeness}} & \multicolumn{2}{c}{\textbf{Reliability}} &
 \multicolumn{2}{c}{\textbf{Engagement}} 
 & \multirow{2}{*}{\textbf{Average}}
\\
\cmidrule(lr){3-5} \cmidrule(lr){6-7} 
\cmidrule(lr){8-9} 
\cmidrule(lr){10-11} 
&  & {\textit{\textbf{Alignment}}} & {\textit{\textbf{Relevance}}} & {\textit{\textbf{Repetition}}} & {\textit{\textbf{Breadth}}}  & {\textit{\textbf{Consistency}}} & {\textit{\textbf{Depth}}} & {\textit{\textbf{Verifiability}}}  & {\textit{\textbf{Engagement}}} & {\textit{\textbf{Novelty}}}   \\
\cmidrule{1-12}
\multicolumn{12}{c}{\cellcolor{grayred} \textbf{\textit{Text as Topic}}} \\
\cmidrule{1-12}
& Direct Gen  & 77.88  &  80.59 & 78.10 &  72.03 & 86.18 &  68.16  &  52.86 &  63.49 &  60.11  & 71.04 \\
& Self-RAG  & 76.08  & 78.34  & 76.60 & 67.07  & 86.14  & 66.19  & 40.51  & 61.97 & 56.99  & 67.77 \\    
& oRAG & 78.92  & 84.97  & 78.98 & 76.05  & 86.38  & 68.83  & 64.61  & 78.60 & 60.29  & 75.29 \\
& Storm  & 72.49  & 71.22  & 69.47 &  65.62 & 79.13 & 62.61 &  52.41 & 58.80  & 55.58  & 65.26   \\
& Co-Storm  & 78.05 & 75.11  & 75.40  & 68.42  & 84.10 &  67.70 &  58.20 & 61.02  & 61.61  & 69.96   \\
& OmniThink & 70.53   & 72.41  & 69.26  &  63.55 & 79.67 & 61.21 &  48.57 & 57.39  & 53.21 & 63.98  \\
& Ours & 81.68 & 88.02  & 83.62 & 79.64 & 90.87 &  73.73  & 70.69  & 71.14  & 69.21  & 78.73   \\
\cmidrule{1-12}
\multicolumn{12}{c}{\cellcolor{uclagold} \textbf{\textit{Image as Topic}}} \\
\cmidrule{1-12}
& Direct Gen &  48.67 & 50.97  & 53.18 &  45.69 & 62.98 &  43.51 &  33.49 & 43.14  &  37.78 & 46.60  \\
& Self-RAG &  57.74 & 50.39  & 66.58 & 42.65  & 78.55  & 51.64  & 26.23  & 42.66 & 44.12 & 51.17  \\
& oRAG &  55.80 & 54.92  & 61.69 & 49.60  & 71.40  & 49.72  & 47.89  & 44.32 & 43.26 & 53.18  \\
& Storm  & 45.80 &  45.99 & 46.38 &  42.69 & 59.60 &  39.92 & 34.23 & 42.38  & 35.17  & 43.57    \\
& Co-Storm  & 47.00 & 44.85  & 47.76 &  41.98 & 61.40 &  41.83  &  35.03 &  41.99 & 37.69 & 44.39   \\
& OmniThink & 43.61 & 43.03  & 45.67 & 38.63  & 58.29 & 42.26 &  29.18 & 38.31  & 33.57 & 41.39   \\
& Ours & 82.57  &  87.20 & 80.22 &  77.24 & 88.75 & 74.99 & 68.41 &  69.36 & 68.69 & 77.49    \\
\cmidrule{1-12}
\multicolumn{12}{c}{\cellcolor{uclablue} \textbf{\textit{Image-Text as Topic}}} \\
\cmidrule{1-12}
& Direct Gen  &  74.63 &  78.73 & 75.43 &  70.16 & 83.66 &  65.78 & 50.53 & 62.36 & 57.73  & 68.78   \\
& Self-RAG  & 72.46  &  70.29 & 74.71 & 59.68  & 84.14  &  63.11 & 37.26  & 57.76 & 54.33 & 63.75  \\
& oRAG & 77.22  & 83.30  & 77.09 & 74.44  & 84.65  & 67.23  & 63.38  & 64.23 & 58.70 & 72.25  \\
& Storm  & 67.20  &  66.64 & 64.33 &  61.61 & 75.29 &  58.26 & 49.21 & 56.25  & 51.27  & 61.12   \\
& Co-Storm  & 70.15  & 67.31  & 68.89 &  61.90 & 79.29 & 61.22  & 52.44   & 57.05  & 55.68 & 63.77 \\
& OmniThink &  64.56 & 64.63  & 63.64  & 57.44  & 75.33 & 56.38 & 43.04 & 54.14  &  48.86 & 58.67  \\
& Ours &  85.26 & 88.44  & 82.11 &  79.31 & 90.63 & 75.20 & 68.59  & 68.79  & 71.06 & 78.82 \\
\bottomrule
\end{tabular}}
\vspace{-5mm}
\end{table*}

==> Tabletex/opensource.tex <==
\begin{table}[h!]
\centering
\vspace{-0.3cm}
\resizebox{0.92\linewidth}{!}{
    \begin{tabular}{c l ccc ccc ccc c}
    \toprule
    \multirow{3}{*}{\textbf{Model}} & \multirow{3}{*}{\textbf{Method}} 
    & \multicolumn{3}{c}{\textbf{Text as Topic}} 
    & \multicolumn{3}{c}{\textbf{Image as Topic}}  
    & \multicolumn{3}{c}{\textbf{Image-Text as Topic}}  & \multirow{3}{*}{\textbf{Average}} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}  \cmidrule(lr){9-11}
    &  & Easy & Medium & Hard & Easy & Medium & Hard & Easy & Medium & Hard \\
    \midrule
    \multirow{5}{*}{Qwen2.5-VL 72B}   
    & oRAG         & 66.22 & 67.15 & 67.07 & 59.09 & 54.92 & 53.74 & 78.09 & 69.01 & 77.12 & 65.34 \\
    & Storm        & 75.95 & 79.21& 73.33 & 69.27 & 65.47 & 63.01& 73.41 & 73.02& 74.55 & 71.92\\
    & Co-Storm     & 80.95 & 79.03 & 82.11 & 64.58 & 65.08 & 72.19 & 80.01 & 78.82 & 79.44 & 75.80 \\
    & OmniThink    & 74.97 & 72.83 & 71.89 & 67.13 & 64.01 & 66.77 & 76.93 & 77.07 & 74.03 & 71.75 \\
    \rowcolor{lightyellow}
    & \textbf{Ours} & \textbf{88.93} & \textbf{85.27} & \textbf{85.08} & \textbf{82.67} & \textbf{81.93} & \textbf{81.67} & \textbf{85.91}  &\textbf{ 87.95} & \textbf{86.26} & \textbf{85.07} \\
    \midrule
    \textbf{GPT-4o} & \textbf{Ours} & 88.51 & 87.53 & 89.71  & 89.07 &89.53 & 90.03  &88.62  & 89.26 & 88.79 & 89.01  \\
    % \multirow{5}{*}{Qwen2.5-VL 7B}   
    % & oRAG         & 27.86 &29.23 &30.72 &30.22 & 27.97 &35.72 & 41.09& 42.85& 38.97 & 33.84 \\
    % & Storm        & 40.83 & 39.92 & 41.07 & 30.27 & 29.77 & 32.19 & 49.61 & 47.70 & 48.95 & 40.04\\
    % & Co-Storm     & 41.09 & 42.73 & 39.85 & 32.07 & 27.98 & 29.04 & 39.77& 41.98 & 40.02& 37.17 \\
    % & OmniThink    & 32.09 & 29.29& 30.18 & 34.03 & 32.79 & 34.77 & 40.92 & 40.92& 36.88 & 34.65 \\
    % \rowcolor{lightyellow}
    % & \textbf{Ours} & \textbf{59.04} & \textbf{56.88} &\textbf{57.20} & \textbf{50.92} & \textbf{49.67} &  \textbf{51.22}  &\textbf{55.08}  & \textbf{57.22} & \textbf{56.02}  & \textbf{54.80}\\
    \bottomrule
    \end{tabular}
}
\vspace{-0.3cm}
\caption{Results in open-source models with Prometheus2.}
\vspace{-0.5cm}
\label{tab:opensource}
\end{table}



